Exploiting Linear Structure Within Convolutional Networks for Efficient Evaluation

We present techniques for speeding up the test-time evaluation of large convolutional networks, designed for object recognition tasks. These models deliver impressive accuracy but each image evaluation requires millions of floating point operations, making their deployment on smartphones and Internet-scale clusters problematic. The computation is dominated by the convolution operations in the lower layers of the model. We exploit the linear structure present within the convolutional filters to derive approximations that significantly reduce the required computation. Using large state-of-the-art models, we demonstrate we demonstrate speedups of convolutional layers on both CPU and GPU by a factor of 2x, while keeping the accuracy within 1% of the original model.

==> fine_tunning.tex <==
\subsection{Fine-tunning}\label{sec:fine_tunning}

Presented methods were applied to fully trained networks. Obviously, networks were not trained
with constrains on connectivity or sparsity as are present in approximated network. This means 
that agresive approximations, which can have much larger speedup are likely to give worse error score. 
Training with new connectivity or sparsity constraint might be quite difficult. Constrains 
comming from approximation would have to be included in optimization, and a lot of additional coding would be
neccessary. We propose different strategy. 


It is easy to decompose weights using any of our method, and then reconstruct them. Particularly,
reconstructed weights can be approximated exactly with the same decomposition. Let's call this process
projection. Proposed strategy is to take a fully trained network, and iterativelly repeat (1) apply projection, 
(2) train for few epochs. Hopefuly, this way weights will become expressable in desired way, which can be speededup
more than $2$ times, and prediction score would be preserved due to fine-tunning. From engineering perspective
stage (1) can be implemented in any external easy environment (e.g. MATLAB), while stage can stay as it is. 
Stage (1) is executed every few epochs, so it is not a computational bottle-neck.

